Moment Matching for Multi-Source Domain Adaptation

Conventional unsupervised domain adaptation (UDA) assumes that training data are sampled from a single domain. This neglects the more practical scenario where training data are collected from multiple sources, requiring multi-source domain adaptation. We make three major contributions towards addressing this problem. First, we collect and annotate by far the largest UDA dataset, called DomainNet, which contains six domains and about 0.6 million images distributed among 345 categories, addressing the gap in data availability for multi-source UDA research. Second, we propose a new deep learning approach, Moment Matching for Multi-Source Domain Adaptation M3SDA, which aims to transfer knowledge learned from multiple labeled source domains to an unlabeled target domain by dynamically aligning moments of their feature distributions. Third, we provide new theoretical insights specifically for moment matching approaches in both single and multiple source domain adaptation. Extensive experiments are conducted to demonstrate the power of our new dataset in benchmarking state-of-the-art multi-source domain adaptation methods, as well as the advantage of our proposed model. Dataset and Code are available at \url{http://ai.bu.edu/M3SDA/}.

==> theory.tex <==
We first motivate our approach from a theoretical perspective.
Following~\cite{ben2010theory}, we introduce a rigorous model of multi-source domain adaptation for binary classification. A domain $\gD=(\mu, f)$ is defined by a probability measure (distribution) $\mu$ on the input space $\gX$ and a labeling function $f:\gX\to[0,1]$ which can be either deterministic or stochastic. 
A hypothesis is a function $h:\gX\to\{0,1\}$.
The probability that a hypothesis $h$ disagrees with the domain labeling function $f$ under the domain distribution $\mu$ is defined as
\begin{equation}
\label{eq_def_error}
    \epsilon_{\gD}(h)=\epsilon_{\gD}(h,f)=\E_{\mu}\big[|h(\vx)-f(\vx)|\big].
\end{equation}

For a source domain $\gD_S$ and a target domain $\gD_T$, we refer to the source error and the target error of a hypothesis $h$ as $\epsilon_S(h)=\epsilon_{\gD_S}(h)$ and $\epsilon_T(h)=\epsilon_{\gD_T}(h)$ respectively.
When the expectation in Equation~\ref{eq_def_error} is computed with respect to an empirical distribution, we denote the corresponding empirical error by $\hat{\epsilon}_{\gD}(h)$, such as $\hat{\epsilon}_S(h)$ and $\hat{\epsilon}_T(h)$.

\begin{definition}[Multi-Source Domain Adaptation]
\label{def:msda}
Given $\gD_{S} = \{\gD_1, \gD_2, ... , \gD_N\}$ the collection of labeled source domains and $\gD_T$ the unlabeled target domain, where all domains are defined by bounded rational measures on input space $\gX$, the multi-source domain adaptation problem aims to find a hypothesis in the given hypothesis space $\gH$, which minimizes the testing target error on $\gD_T$.
\end{definition}

In order to analyze the target error for multi-source domain adaptation algorithms, it is important to measure the difference between the source domains and the target domain. In contrast with existing theoretical analysis on domain adaptation~\cite{ben2010theory, Zhao2017MultipleSD, NIPS2007_3212} that is based on a divergence measure known as the $\mathcal{H}$-divergence, we introduce the following definition of cross-moment divergence.
\begin{definition}[cross-moment divergence]
\label{def:cmomentdiv}
Given a compact domain $\gX\subset\R^n$ and two probability measures $\mu,\mu'$ on $\gX$, the $k$-th order cross-moment divergence between $\mu$ and $\mu'$ is
\begin{equation*}
\begin{split}
    & \ d_{CM^k}(\mu,\mu')\\
   =& \sum_{\rvi\in\Delta_k}
    	\Bigg|\int_{\gX}\prod_{j=1}^n(x_j)^{i_j}d\mu(x) 
      -\int_{\gX}\prod_{j=1}^n(x_j)^{i_j}d\mu'(x)\Bigg|,
\end{split}
\end{equation*}
where $\Delta_k=\{(i_1,i_2,\ldots,i_n)\in\N^n_0|\sum_{j=1}^ni_j=k\}$.
\end{definition} 

Ben-David \textit{et al}\cite{ben2010theory} provide target error bounds for learning from multiple sources, based on $\mathcal{H}$-divergence, \ie, a symmetric difference measure between the target and source domains \textit{w.r.t.} a hypothesis class $\mathcal{H}$. Following the same setup, we provide similar bounds based on the pairwise cross-moment divergence between target and source domains.

In the multi-source settings, a learning algorithm is presented with training sets from each of the $N$ source domains and learns a model that performs well on the target domain. In particular, we examine algorithms that minimize convex combinations of source errors, i.e., given a weight vector $\valpha=(\alpha_1,\ldots,\alpha_N)$ with $\sum_{j=1}^N\alpha_j=1$, we define the $\valpha$-weighted source error of hypothesis $h$ as
\[\epsilon_{\valpha}(h)=\sum_{j=1}^N\alpha_j\epsilon_j(h),\]
where $\epsilon_j(h)$ is the shorthand of $\epsilon_{\gD_j}(h)$. The empirical $\valpha$-weighted source error can be defined analogously and denoted by $\hat{\epsilon}_{\valpha}(h)$.

\begin{restatable}{theorem}{pairwisebound}
\label{thm:pairwise_bound}
Let $\gH$ be a hypothesis space of $VC$ dimension $d.$ For each $\gD_j\in\{\gD_1, \gD_2, ... , \gD_N\}$, let $S_j$ be a labeled sample set of size $\beta_jm$ drawn from $\mu_j$ and labeled by the groundtruth labeling function $f_j.$ If $\hat{h}\in\gH$ is the empirical minimizer of $\hat{\epsilon}_{\valpha}(h)$ for a fixed weight vector $\valpha$ and $h^*_T=\min_{h\in\gH}\epsilon_T(h)$ is the target error minimizer, then for any $\delta\in(0,1)$ and any $\epsilon>0$, there exist $N$ integers $\{n^j_\epsilon\}_{j=1}^N$ and $N$ constants $\{a_{n^j_\epsilon}\}_{j=1}^N$, such that with probability at least $1-\delta,$

\begin{equation}
\label{eqn:pair_bound}
\begin{split}
\epsilon_T(\hat{h})\leq& \ \epsilon_T(h^*_T)+\eta_{\valpha,\vbeta,m,\delta}
	+ \epsilon \\
	&+ \sum_{j=1}^N\alpha_j\bigg(2\lambda_j+a_{n^j_\epsilon}\sum_{k=1}^{n^j_\epsilon}d_{CM^{k}}\big(\gD_j, \gD_T\big)\bigg),
\end{split}
\end{equation}
where $\eta_{\valpha,\vbeta,m,\delta} = 4\sqrt{\Big(\sum_{j=1}^{N} \frac {\alpha_{j}^2} {\beta_{j}} \Big) \Big(\frac {2d(\log(\frac{2km}{d})+1)+2\log(\frac{4}{\delta})} {km}\Big) },$
$k=\sum_{j=1}^N\beta_{j},$
and $\lambda_j=\min_{h\in\gH}\{\epsilon_T(h)+\epsilon_j(h)\}.$
\end{restatable}

\begin{proof}
See \textit{\url{Appendix}}.
\end{proof}

Theorem~\ref{thm:pairwise_bound} shows that the upper bound on the target error of the learned hypothesis depends on the pairwise moment divergence $d_{CM^{k}}\big(\gD_S,\gD_T\big)$ between the target domain and each source domain. This motivates our method for multi-source domain adaptation to align the moments between each target-source pair. 
Moreover, it is obvious that the last term of the bound, $\sum_{k}d_{CM^{k}}\big(\gD_j, \gD_T\big)$, is lower bounded by the pairwise divergences between source domains. To see this, consider the toy example consisting of two sources $\gD_1,\gD_2$ and a target $\gD_T,$ since $d_{CM^{k}}(\cdot,\cdot)$ is a metric, triangle inequality implies
$$d_{CM^{k}}\big(\gD_1, \gD_T\big) + d_{CM^{k}}\big(\gD_2, \gD_T\big)
\geq d_{CM^{k}}\big(\gD_1, \gD_2\big).$$
This motivates our algorithm to also align the moments between each pair of source domains. Given computational concerns, our algorithm adopts the following $L$-2 norm moment distance up to the second order instead of the cross-moment divergence.\footnote{This can be regarded as an approximation of the second order cross-moment matrix by its trace.}
\vspace{-0.2cm}

==> tmp.tex <==
\section{1}
\section{2}
\section{3}
\section{4}
\section{5}
\section{7}
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage
1
\clearpage

\begin{equation}
\label{eqn:MD2}
    sfsf
\end{equation}
\begin{equation}
    sfsf
\end{equation}
\begin{equation}
    sfsf
\end{equation}
\begin{equation}
    sfsf
\end{equation}
\begin{equation}
    sfsf
\end{equation}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_digit_five_1}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_digit_five}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_challengeI}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_digit_five_4}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_digit_five_5}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab_digit_five_6}
\end{table}


\begin{figure}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics{}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

\begin{restatable}{theorem}{pairwisebound}
\label{thm:pairwise_bound}
Let $\gH$ be a hypothesis space of $VC$ dimension $d.$ Let $m$ be the size of labeled samples from all sources $\{\gD_1, \gD_2, ... , \gD_N\}$, $S_j$ be the labeled sample set of size $\beta_jm$ ($\sum_j\beta_j=1$) drawn from $\mu_j$ and labeled by the groundtruth labeling function $f_j.$ If $\hat{h}\in\gH$ is the empirical minimizer of $\hat{\epsilon}_{\valpha}(h)$ for a fixed weight vector $\valpha$ and $h^*_T=\min_{h\in\gH}\epsilon_T(h)$ is the target error minimizer, then for any $\delta\in(0,1)$ and any $\epsilon>0$, there exist $N$ integers $\{n^j_\epsilon\}_{j=1}^N$ and $N$ constants $\{a_{n^j_\epsilon}\}_{j=1}^N$, such that with probability at least $1-\delta,$

\begin{equation}
\label{eqn:pair_bound}
\begin{split}
\epsilon_T(\hat{h})\leq& \ \epsilon_T(h^*_T)+\eta_{\valpha,\vbeta,m,\delta}
	+ \epsilon \\
	&+ \sum_{j=1}^N\alpha_j\bigg(2\lambda_j+a_{n^j_\epsilon}\sum_{k=1}^{n^j_\epsilon}d_{CM^{k}}\big(\gD_j, \gD_T\big)\bigg),
\end{split}
\end{equation}
where $\eta_{\valpha,\vbeta,m,\delta} = 4\sqrt{\Big(\sum_{j=1}^{N} \frac {\alpha_{j}^2} {\beta_{j}} \Big) \Big(\frac {2d(\log(\frac{2m}{d})+1)+2\log(\frac{4}{\delta})} {m}\Big) }$
%$k=\sum_{j=1}^N\beta_{j},$
and $\lambda_j=\min_{h\in\gH}\{\epsilon_T(h)+\epsilon_j(h)\}.$
\end{restatable}
